Hidden Entity Detection from GitHub Leveraging Large Language Models

Named entity recognition is an important task when constructing knowledge bases from unstructured data sources. Whereas entity detection methods mostly rely on extensive training data, Large Language Models (LLMs) have paved the way towards approaches that rely on zero-shot learning (ZSL) or few-shot learning (FSL) by taking advantage of the capabilities LLMs acquired during pretraining. Specifically, in very specialized scenarios where large-scale training data is not available, ZSL / FSL opens new opportunities. This paper follows this recent trend and investigates the potential of leveraging Large Language Models (LLMs) in such scenarios to automatically detect datasets and software within textual content from GitHub repositories. While existing methods focused solely on named entities, this study aims to broaden the scope by incorporating resources such as repositories and online hubs where entities are also represented by URLs. The study explores different FSL prompt learning approaches to enhance the LLMs' ability to identify dataset and software mentions within repository texts. Through analyses of LLM effectiveness and learning strategies, this paper offers insights into the potential of advanced language models for automated entity detection.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> table-classification-trainlen60.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
        \hline\rule{0pt}{12pt}
         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\makecell{Evaluation \\  Setting}}} & %\multicolumn{2}{c}{\textbf{zero-shot}} & 
         \multicolumn{4}{c}{\textbf{Static Few-shot}}  &
         \multicolumn{4}{c}{\textbf{Dynamic Few-shot}}\\
         & & \textbf{P} & \textbf{R} & 
         \textbf{P(b}) & \textbf{R(b)} & 
         \textbf{P} & \textbf{R} & 
         \textbf{P(b)} & \textbf{R(b)}\\
         \hline\rule{0pt}{12pt}
         \multirow{4}{*}{Llama 2 7b  } & Strict & 0.400 & 0.445 & 0.613 & 0.682 & 0.292 &0.310 &0.607 &0.646\\
         & Exact &0.873
         & 0.971& 0.873 & 0.971 &0.891&0.949&0.891&0.949\\
         & Partial & 0.873& 0.971& 0.873 & 0.971 &
         0.892&0.950&0.892&0.950\\
         & Type & 0.411& 0.457& 0.629 & 0.700 &
         0.303&0.322&0.622&0.662\\
         \hline\rule{0pt}{12pt}
         \multirow{4}{*}{\makecell{Llama 2 7b \\  qt4bit }} & Strict & 0.295& 0.360& 0.519 &0.629 &
         0.306&0.377&0.535&0.663\\
         & Exact  &0.697 &0.852 &0.794  &0.852 &
         0.706&0.871&0.703&0.872\\
         & Partial  & 0.708& 0.866& 0.715 &0.866 &
         0.717&0.884&0.714&0.886\\
         & Type & 0.325& 0.397&0.580 &0.702 &
         0.329&0.406&0.589&0.730\\
         \hline\rule{0pt}{12pt}
         \multirow{4}{*}{Mistral 7b}& Strict  & 0.466&0.503 & 0.692 & 0.747&
         0.512&0.5554&0.720&0.779 \\
         & Exact  &0.860 & 0.928 &0.860 & 0.928
         &0.874&0.945&0.874&0.945\\
         & Partial  & 0.860&0.928 &0.860 & 0.928&
         0.874&0.945&0.874&0.945\\
         & Type  & 0.478&0.516 & 0.719& 0.776&
         0.524&0.567&0.751&0.812\\
         \hline\rule{0pt}{12pt}
         \multirow{4}{*}{\makecell{Mistral 7b \\  qt4bit }} & Strict & 0.434&0.458 &0.646 &0.666 &
         0.419&0.457&0.626&0.665\\
         & Exact  &0.781 &0.823 &0.801  &0.826 &
         0.770&0.841&0.792&0.842\\
         & Partial  &0.791 &0.835 &0.801  &0.826 &
         0.778&0.849&0.799&0.850\\
         & Type &0.473 &0.499 &0.698 & 0.720&
         0.454&0.496&0.683&0.726\\
         \hline\rule{0pt}{12pt}
    \end{tabular}
    \caption{Performance of different LLMs for dataset URL annotation as classification task.}
    \label{tab:my_label}
\end{table}


==> table-extraction-trainlen60.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
        \hline\rule{0pt}{12pt}
         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\makecell{Evaluation \\  Setting}}} & %\multicolumn{2}{c}{\textbf{zero-shot}} & 
         \multicolumn{4}{c}{\textbf{Static Few-shot}}  &
         \multicolumn{4}{c}{\textbf{Dynamic Few-shot}}\\
         & & \textbf{P} & \textbf{R} & 
         \textbf{P(b}) & \textbf{R(b)} & 
         \textbf{P} & \textbf{R} & 
         \textbf{P(b)} & \textbf{R(b)}\\
         \hline\rule{0pt}{12pt}
         \multirow{4}{*}{Llama 2 7b  } & Strict & 0.373 & 0.486 & 0.477 & 0.630 &
         0.267 &0.331 &0.510 &0.637\\
         & Exact &0.701 & 0.914& 0.693 & 0.914 & 0.723&0.895&0.717&0.895\\
         & Partial & 0.706& 0.921& 0.698 & 0.921 &0.727&0.901&0.722&0.901\\
         & Type & 0.391& 0.510& 0.506 & 0.668 &0.284&0.352&0.539&0.673\\
         \hline\rule{0pt}{12pt}
         \multirow{4}{*}{\makecell{Llama 2 7b \\  qt4bit }} & Strict &0.357&0.375 &0.572 &0.604&
         0.319&0.367&0.568&0.670\\
         & Exact  &0.788 &0.829 &0.786  &0.829 &
         0.788&0.829&0.786&0.829\\
         & Partial  &0.801 &0.841 &0.798  &0.841 &
         0.801&0.841&0.798&0.841\\
         & Type &0.386 &0.405 &0.630 &0.665 &
         0.386&0.405&0.630&0.665\\
         \hline\rule{0pt}{12pt}
         \multirow{4}{*}{Mistral 7b}& Strict  & 0.506&0.478 & 0.704 & 0.665&
         0.517&0.513&0.720& 0.716 \\
         & Exact  &0.876 & 0.828 &0.876 & 0.828&
         0.874 & 0.869&0.873&0.869\\
         & Partial  & 0.879&0.831 &0.879 & 0.831&
         0.876&0.871&0.875&0.871\\
         & Type  & 0.521&0.492 & 0.749& 0.708&
         0.534&0.530&0.762&0.759\\
         \hline\rule{0pt}{12pt}
         \multirow{4}{*}{\makecell{Mistral 7b \\  qt4bit }} & Strict & 0.451& 0.440&0.664  &0.648 &
        0.422 &0.414&0.634&0.621\\
         & Exact  & 0.831& 0.811&0.832  & 0.811&
         0.805&0.790&0.806&790\\
         & Partial  &0.836 &0.815 & 0.836 &0.816 &
         0.813&0.797&0.814&0.797\\
         & Type &0.478 &0.466 &0.707 &0.690 &
         0.448&0.439&0.687&0.673\\
         \hline\rule{0pt}{12pt}
    \end{tabular}
    %\caption{Performance of different LLMs for dataset URL annotation as extraction task.}
    \caption{Performance of different LLMs for the E+CL task.}
    \label{tab:e+cl}
\end{table}

